Gamma factors for Asai representations of ${\rm GL}_2$

Let $E$ be a quadratic semisimple extension of a local field $F$ of characteristic zero. We determine explicit relation between gamma factors for Asai representations of $R_{E/F}{\rm GL}_{2/E}$ defined by the Weil-Deligne representations and local zeta integrals. When $E = F\times F$, the results were due to Henniart and Jacquet. We completed the theory in this article based on explicit calculation.

==> amssymbol.tex <==
\usepackage{amsmath}
\usepackage{amscd,amsthm,amssymb,amsfonts}
\usepackage{mathrsfs}
\usepackage{dsfont}
\usepackage{stmaryrd}
\usepackage{euscript}
\usepackage{expdlist}
\usepackage{enumerate}

%\usepackage{enumitem}
%\usepackage[mathscr]{eucal}
% either use \mathscr (no euscript package), or use \EuScript (no eucal
% package), they are the same font
%\input xy
%\xyoption{all}
\setlength{\topmargin}{-0.4in}
\setlength{\headheight}{8pt} \setlength{\textheight}{9in}
\setlength{\oddsidemargin}{-0.15in}
\setlength{\evensidemargin}{-0.15in} \setlength{\textwidth}{6.6in}
%\usepackage[OT2,T1]{fontenc}

% newcommands for thesis
%\renewcommand{\thesubsubsection}{\thesubsubsection}
%\newcommand{\mysubsection}[1]{\subsection[#1]{\normalfont\itshape #1}}
%\def\subsubsection{\@startsection{subsubsection}{3}{\z@}{-3.25ex plus -1ex minus -.2ex}{1.5ex plus .2ex}{\normalsize\itshape}}
%\newcommand{\mysubsubsection}{\subsubsection}
% theorems, lemmas,..
\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
%\renewcommand{thethm}{\arabic{section}.\arabic{subsection}}
\newtheorem{thmA}{Theorem}
\renewcommand{\thethmA}{\Alph{thmA}}
\newtheorem{corA}{Corollary}
\renewcommand{\thecorA}{\Alph{thmA}}
\newtheorem{hypA}{Hypothesis}
\renewcommand{\thehypA}{\Alph{hypA}}
\newtheorem{assumption}[thm]{Assumption}
\newtheorem*{thma}{Theorem A}
\newtheorem*{thmb}{Theorem B}
\newtheorem*{thmc}{Theorem C}
\newtheorem*{thmd}{Theorem D}
\newtheorem*{thm*}{Theorem}
\newtheorem*{say}{Say}
\newtheorem{lm}[thm]{Lemma}
\newtheorem{cor}[thm]{Corollary}
\newtheorem*{cor*}{Corollary}
\newtheorem{prop}[thm]{Proposition}
\newtheorem*{conj*}{Conjecture}
\newtheorem{conj}{Conjecture}

%proposal
\newtheorem{expected_thm}{Expected theorem}
\newtheorem{consequence}{Consequence}

\newtheorem{I_thm}{Theorem} % Used in Introduction
\newtheorem{I_cor}{Corollary} % Used in Introduction

\theoremstyle{remark}
\newtheorem*{remark}{Remark}
\newtheorem{I_remark}{Remark} % Used in Introduction
\newtheorem*{thank}{Acknowledgments}
\newtheorem*{Notation}{Notation}

\theoremstyle{definition}
\newtheorem{I_defn}{Definition} % Used in Introduction
\newtheorem*{defn*}{Definition}
\newtheorem{Remark}[thm]{Remark}
\newtheorem{I_Remark*}{Remark}
\newtheorem{defn}[thm]{Definition}
\newtheorem{EX}{Exercise}
\newtheorem{example}[thm]{Example}
\newtheorem{problem}{Problem}

\newtheorem{hypothesis}[thm]{Hypothesis}
\newtheorem*{hypR}{Hypothesis R}
\renewcommand{\thehypothesis}{\Alph{hypothesis}}


%for temporary use
\newcommand{\nc}{\newcommand}
\newcommand{\renc}{\renewcommand}

%Convenient command
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bpmx}{\begin{pmatrix}}
\newcommand{\epmx}{\end{pmatrix}}
\newcommand{\bbmx}{\begin{bmatrix}}
\newcommand{\ebmx}{\end{bmatrix}}
\newcommand{\wh}{\widehat}
\newcommand{\wtd}{\widetilde}
\newcommand{\thetalift}[2]{\theta_{#1}(#2)}
%\newcommand{\bsp}{\begin{split}}



%\newcommand{\esp}{\end{split}}
\newcommand{\beqcd}[1]{\begin{equation*}\label{#1}\tag{#1}}
\newcommand{\eeqcd}{\end{equation*}}
\renewcommand{\theequation}{\thesection\thesubsection\thesubsubsection.\arabic{equation}}
\numberwithin{equation}{section}
\newenvironment{mylist}{
  \begin{enumerate}{}{%
      \setlength{\itemsep}{5pt} \setlength{\parsep}{0in}
      \setlength{\parskip}{0in} \setlength{\topsep}{0in}
      \setlength{\partopsep}{0in}
      \setlength{\leftmargin}{0.17in}}}{\end{enumerate}}

\newenvironment{myP}{
  \begin{description}[\breaklabel\setlabelstyle{\bfseries}]}{\end{description}}


% references
\def\parref#1{\ref{#1}}
\def\thmref#1{Theorem~\parref{#1}}
\def\expectthmref#1{Expected theorem~\parref{#1}}
\def\propref#1{Proposition~\parref{#1}}
\def\corref#1{Corollary~\parref{#1}}     \def\remref#1{Remark~\parref{#1}}
\def\secref#1{\S\parref{#1}}
\def\chref#1{Chapter~\parref{#1}}
\def\lmref#1{Lemma~\parref{#1}}
\def\subsecref#1{\S\parref{#1}}
\def\defref#1{Definition~\parref{#1}}
\def\assref#1{Assumption~\parref{#1}}
\def\hypref#1{Hypothesis~\parref{#1}}
\def\subsubsecref#1{\S\parref{#1}}
\def\egref#1{Example~\parref{#1}}
\def\exref#1{Exercise~\parref{#1}}
\def\conjref#1{Conjecture~\parref{#1}}
\def\makeop#1{\expandafter\def\csname#1\endcsname
  {\mathop{\rm #1}\nolimits}\ignorespaces}
%\def\thmref#1{Theorem\hyperref[#1]{\ref{#1}}}

\newenvironment{list2}{
  \begin{list}{$\bullet$}{%
      \setlength{\itemsep}{0in}
      \setlength{\parsep}{0in} \setlength{\parskip}{0in}
      \setlength{\topsep}{0in} \setlength{\partopsep}{0in}
      \setlength{\leftmargin}{0.2in}}}{\end{list}}




%Reserved Key words
\makeop{Hom}   \makeop{End}   \makeop{Aut}   %\makeop{Isom}
\makeop{Pic} \makeop{Gal}       \makeop{Div} \makeop{Lie}
\makeop{PGL}   \makeop{Corr} \makeop{PSL} \makeop{sgn} \makeop{Spf}
 \makeop{Tr} \makeop{Nr} \makeop{Fr} \makeop{disc}
\makeop{Proj} \makeop{supp} \makeop{ker}   \makeop{Im} \makeop{dom}
\makeop{coker} \makeop{Stab} \makeop{SO} \makeop{SL} \makeop{SL}
\makeop{Cl}    \makeop{cond} \makeop{Br} \makeop{inv} \makeop{rank}
\makeop{id}    \makeop{Fil} \makeop{Frac}  \makeop{GL} \makeop{SU}
\makeop{Trd}   \makeop{Sp} \makeop{Tr}    \makeop{Trd} \makeop{Res}
\makeop{ind} \makeop{depth} \makeop{Tr} \makeop{st} \makeop{Ad}
\makeop{Int} \makeop{tr}    \makeop{Sym} \makeop{can} \makeop{SO}
\makeop{torsion} \makeop{GSp} \makeop{Tor}\makeop{Ker} \makeop{rec}
\makeop{Ind} \makeop{Coker}
 \makeop{vol} \makeop{Ext} \makeop{gr} \makeop{ad}
 \makeop{Gr}\makeop{corank} \makeop{Ann}
\makeop{Hol} %Holomorphic
\makeop{Fitt} \makeop{Mp} \makeop{CAP}
\def\Jac{\mathrm{Jac}}
%\makeop{Sel}
\def\Sel{Sel}
\def\ord{{ord}}
\def\Isom{\ul{\mathrm{Isom}}}
\def\Inj{\ul{\mathrm{Inj}}}
\def\Ord{{\mathrm{ord}}}
%\def\Ord{{\operatorname{ord}}}
\def\Cov{\mathrm{Cov}}
\def\Imb{\mathrm{I}}
\def\cusp{{\mathrm{cusp}}}

%GU(3,3)
\DeclareMathOperator{\GO}{GO}
\DeclareMathOperator{\GSO}{GSO}
\def\Gsp{{\rm Gsp}}
\def\PGsp{{\rm PGsp}}
\def\MSL{\widetilde{\SL}}
%\def\GO{{\rm GO}}
%\def\GSO{{\rm GSO}}

%\DeclareMathOperator{\Spec}{Spec}
\def\Spec{\mathrm{Spec}\,}
\DeclareMathOperator{\Eis}{Eis}
\DeclareMathOperator{\codim}{codim}
\DeclareMathOperator{\length}{length}
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}
%\DeclareSymbolFont{cyrletters}{OT2}{wncyr}{m}{n}
%\DeclareMathSymbol{\SHA}{\mathalpha}{cyrletters}{"58}



\def\makebb#1{\expandafter\def
  \csname bb#1\endcsname{{\mathbb{#1}}}\ignorespaces}
\def\makebf#1{\expandafter\def\csname bf#1\endcsname{{\bf
      #1}}\ignorespaces}
\def\makegr#1{\expandafter\def
  \csname gr#1\endcsname{{\mathfrak{#1}}}\ignorespaces}
\def\makescr#1{\expandafter\def
  \csname scr#1\endcsname{{\EuScript{#1}}}\ignorespaces}
\def\makecal#1{\expandafter\def\csname cal#1\endcsname{{\mathcal
      #1}}\ignorespaces}
% \cal is used in article, \mathcal is used in amsart

\def\doLetters#1{#1A #1B #1C #1D #1E #1F #1G #1H #1I #1J #1K #1L #1M
                 #1N #1O #1P #1Q #1R #1S #1T #1U #1V #1W #1X #1Y #1Z}
\def\doletters#1{#1a #1b #1c #1d #1e #1f #1g #1h #1i #1j #1k #1l #1m
                 #1n #1o #1p #1q #1r #1s #1t #1u #1v #1w #1x #1y #1z}
\doLetters\makebb   \doLetters\makecal  \doLetters\makebf
\doLetters\makescr
\doletters\makebf   \doLetters\makegr   \doletters\makegr
\def\pfname{\medbreak\noindent{\scshape Proof.}\enspace}%
\renewcommand{\proofname}{\pfname}
%\def\pf{\proof}
%\def\qed{\qedmark\medbreak}%
%\def\qedmark{{\enspace\vrule height 6pt width 5pt depth 1.5pt}}%

\def\semidirect{\rtimes}    \def\setminus{\smallsetminus}
\def\Gm{{\bbG}_{m}}   \def\Ga{{{\bbG}_{\rm a}}}

\def\formalgm{\widehat{\bbG}_m}
\renewcommand{\baselinestretch}{1.02}\normalsize

\def\der{{\rm der}}
\makeop{Ram} \makeop{Rep} \makeop{mass}

\def\model#1{\underline{#1}}
\def\bfproj{\mathop{\bf Proj}\nolimits}
\def\sep{{\rm sep}}
\makeop{Bl}
\def\abs#1{\left|#1\right|}
\def\norm#1{\lVert#1\rVert}
%\newcommand{\norm}[1]{\left\Vert#1\right\Vert}
%\newcommand{\abs}[1]{\left\vert#1\right\vert}

\def\Fpbar{\bar{\mathbb F}_p}
\def\Fp{{\mathbb F}_p}
\def\Fq{{\mathbb F}_q}
\def\Qlbar{\overline{{\Q}_{\ell}}}
\def\Ql{{\Q}_{\ell}}
\def\Qpbar{\ol{\Q_p}}
\def\Qbarp{\C_p}
\def\Qp{\Q_p}
\def\Qbar{\ol{\Q}}
\def\Zbar{\ol{\Z}}
%\def\Zpbar{\ol{\Z_p}}
\def\Zbarp{\Zbar_p}
\def\Zbarlp{\Zbar_{(p)}}

\def\Zp{\Z_p}
\def\mZbar{\frakm_{\Zbar}}
\def\mZbarp{\frakm_p}
\def\diag#1{\mathrm{diag}(#1)}
\def\el{\ell}
%*************FONTS*****************

\def\Ibar{\overline{I}}
\def\Mbar{\ol{M}}
\def\Sbar{\ol{S}}
\def\Dbar{\ol{D}}
\def\fbar{\bar{f}}
\def\lbar{\bar{l}}
\def\ybar{\bar{y}}
\def\kbar{\bar{k}}
\def\rhobar{\bar{\rho}}
%basic notation

\def\rmT{{\mathrm T}}
\def\rmN{{\mathrm N}}
\def\rmF{{\mathrm F}}
\def\rmC{{\mathrm C}}
\def\rmp{{\mathrm p}}
% mathcal
\def\cA{{\mathcal A}}  %automorphic forms
\def\cB{\EuScript B}
\def\cD{\mathcal D}
\def\cE{{\mathcal E}}
\def\cF{{\mathcal F}}  %Hida family
\def\cG{{\mathcal G}}
\def\cL{{\mathcal L}}
\def\cH{{\mathcal H}}
\def\cI{\mathcal I}
\def\cJ{\mathcal J}
\def\cK{{\mathcal K}}  %imaginary quadratic field
\def\cM{\mathcal M}
\def\cR{{\mathcal R}}
\def\cO{\mathcal O}
\def\cS{{\mathcal S}}
\def\cf{{\mathcal f}}
\def\cW{{\mathcal W}}
\def\ca{{\mathcal a}}
\def\cZ{\mathcal Z}
\def\cX{\mathcal X}
\def\cV{{\mathcal V}}
\def\cP{{\mathcal P}}
\def\cC{\mathcal C}
\def\cJ{\mathcal J}
\def\cN{\mathcal N}
\def\cT{\mathcal T}
\def\cY{\mathcal Y}
\def\cQ{\mathcal Q}
\def\cU{\mathcal U}

\def\calX{\mathcal X}
% EuScript
\def\EucA{{\EuScript A}}
\def\EucB{\EuScript B}
\def\EucD{\EuScript D}
\def\EucE{{\EuScript E}}
\def\EucF{{\EuScript F}}  %Hida family
\def\EucG{{\EuScript G}}
\def\EucL{{\EuScript L}}
\def\EucH{{\EuScript H}}
\def\EucI{\EuScript I}
\def\EucJ{\EuScript J}
\def\EucK{{\EuScript K}}
\def\EucM{{\EuScript M}}
\def\EucR{{\EuScript R}}
\def\EucO{{\EuScript O}}
\def\EucS{{\EuScript S}}
\def\Eucf{{\EuScript f}}
\def\EucW{{\EuScript W}}
\def\EucZ{\EuScript Z}
\def\EucX{\EuScript X}
\def\EucV{{\EuScript V}}
\def\EucP{{\EuScript P}}
\def\EucC{\EuScript C}
\def\EucJ{\EuScript J}
\def\EucN{\EuScript N}
\def\EucT{\EuScript T}
\def\EucY{\EuScript Y}
\def\EucQ{\EuScript Q}
\def\EucU{\EuScript U}



%\mathbf for U(n,n)
\def\bfc{\mathbf c}

\def\bfH{\mathbf H}
\def\bG{\mathbf G}
\def\bI{\mathbf I}
\def\bE{\mathbf E}
\def\bP{\mathbf P}
\def\bfK{\mathbf K}
\def\bN{\mathbf N}
\def\bM{\mathbf M}
\def\bfM{\mathbf M}
\def\bfU{\mathbf U}
\def\bfT{{\mathbf T}}
\def\bfL{\mathbf L}
\def\bda{\mathbf a}
\def\bff{\mathbf f}
\def\bdh{\mathbf h}
\def\bdg{\mathbf g}
\def\bdx{\mathbf x}
\def\bdy{\mathbf y}
\def\bdp{\mathbf p}
\def\bfi{\mathbf i}
\def\bfu{\mathbf u}
\def\bdw{\mathbf w}
\def\bdS{\mathbf S}
\def\bdd{\mathbf d}
\def\bdc{\mathbf c}
\def\bdn{\mathbf n}
\def\bF{\mathbf F}
\def\bD{\mathbf D}
\def\bW{\mathbf W}
\def\bfw{\mathbf w}

%boldsymbol
\def\bfEucJ{\boldsymbol{\EucJ}}
\def\bfeta{\boldsymbol{\eta}}
\def\bflambda{\boldsymbol{\lambda}}
\def\bfrho{\boldsymbol{\rho}}
\def\bfdelta{\boldsymbol{\delta}}
\def\bftheta{\boldsymbol{\theta}}
\def\bfxi{\boldsymbol{\xi}}
\def\bfal{\boldsymbol{\alpha}}
\def\bfvep{\boldsymbol{\varepsilon}}
\def\bfep{\boldsymbol{\ep}}
\def\bfDelta{\boldsymbol{\Delta}}
% mathscr
\def\sG{\mathscr G}
\def\sH{\mathscr H}
\def\sF{\mathscr F}
\def\sL{\mathscr L}
\def\sI{\mathscr I}
\def\sJ{\mathscr J}
\def\sC{\mathscr C}
\def\sX{\mathscr X}
\def\sM{\mathscr M}
\def\sA{\mathscr A}
\def\sV{\mathscr V}
\def\sK{\mathscr K}
\def\sN{\mathscr N}
\def\sD{\mathscr D}
\def\sU{\mathscr U}
\def\sR{\mathscr R}
\def\sB{\mathscr B}
\def\sO{\mathscr O}
\def\sS{\mathscr S}
\def\sP{\mathscr P}
\def\sW{{\mathscr W}}
\def\sT{\mathscr T}
% mathbb
\def\T{{\mathbb T}}
\def\V{\mathbb V} %p-adic modular forms
\def\bbM{\mathbb M}
\def\bbI{\mathbb I}
\def\bbX{\mathbb X}
\def\bbY{\mathbb Y}
\def\bbJ{\mathbb J}
\def\bbL{\mathbb L}
\def\bbS{\mathbb S}
\newcommand{\Z}{\mathbf Z}
\newcommand{\Q}{\mathbf Q}
\newcommand{\R}{\mathbf R}
\newcommand{\C}{\mathbf C}
%\newcommand{\D}{\mathbf D}    % pro algebraic torus
\newcommand{\A}{\mathbf A}    % for adele
\newcommand{\F}{\mathbb F}
\def\bbK{\mathbb K}
\def\bbE{{\mathbb E}}
\def\bbV{\mathbb V}
\def\bbH{\mathbb H}
\def\bbW{\mathbb W}

\def\bbmu{\boldsymbol{\mu}}


% mathfrak
\def\cond{{c}}
\def\gm{{\mathfrak m}}

\def\fraka{{\mathfrak a}}
\def\frakb{{\mathfrak b}}
\def\frakc{{\mathfrak c}}
\def\frakd{\mathfrak d}
\def\frakf{\mathfrak f}
\def\frakk{\mathfrak k}
\def\frakp{{\mathfrak p}}
\def\frakP{\mathfak P}
\def\frakq{\mathfrak q}
\def\frakr{\mathfrak r}
\def\frakt{\mathfrak t}
\def\frakg{\mathfrak g}
\def\frakm{\mathfrak m}
\def\frakn{\mathfrak n}
\def\frakl{\mathfrak l}
\def\frakP{\mathfrak P}
\def\frakF{{\mathfrak F}}
\def\frakE{\mathfrak E}
\def\frakL{{\mathfrak L}}
\def\frakD{\mathfrak D}
\def\frakM{\mathfrak M}
\def\frakG{{\mathfrak G}}
\def\frakh{\mathfrak h}
\def\frakH{{\mathfrak H}}
\def\frakV{\mathfrak V}
\def\frakI{\mathfrak I}
\def\frakA{\mathfrak A}
\def\frakB{\mathfrak B}
\def\frakC{{\mathfrak C}}
\def\frakJ{\mathfrak J}
\def\frakX{\mathfrak X}
\def\frako{\mathfrak o}
\def\frakQ{\mathfrak Q}
\def\fraks{\mathfrak s}
\def\frakR{\mathfrak R}
\def\frakS{\mathfrak S}
\def\frakW{\mathfrak W}
\def\frakN{\mathfrak N}
\def\il{\mathfrak i\frakl}
\def\fraki{\mathfrak i}
\def\frakz{\mathfrak z}
%\mathpzc
\def\pzcw{\mathpzc w}
\def\pzcv{\mathpzc v}


% one
\def\bfone{{\mathbf 1}}
\def\bfzero{\mathbf 0}
\def\one{\mathbf 1} %trivial character

% underline
\def\ulA{\ul{A}}
\def\ulV{\ul{V}}
\def\ulW{\ul{W}}
\def\ulx{\ul{x}}
\def\ulN{\ul{N}}
\def\ulz{\ul{z}}
\def\ula{\ul{a}}
\def\nv{{\underline n}}

\def\ollam{\bar{\lam}}

%widetilde
\def\wtcG{\widetilde{\cG}}
\def\wtG{\widetilde{G}}
\def\wtE{\widetilde{E}}

%widehat
\def\whG{\widehat{G}}
\def\whX{\widehat{\chi}}
\def\whE{\widehat{E}}

%*********bar
\def\Vbar{\ol{V}}
\def\xbar{\ol{x}}
\def\ibar{\bar{i}}
\def\abar{\bar{a}}
\def\Hbar{\ol{H}}
\def\Zhat{\widehat{\Z}}
\def\wbar{\bar{w}}
\def\cSbar{\ol{\cS}}
\def\vbar{\bar{v}}
\def\wbar{\ol{w}}
\def\zbar{\ol{z}}


%******************French words
\def\et{{\acute{e}t}}

%****************** long words
%\def\SHA{\mathrm{III}}
\def\ac{algebraically closed }
\def\dieu{Dieudonn\'{e} }
\def\ab{abelian variety }
\def\etale{{\'{e}tale }}
%\newcommand{\abs}{abelian varieties }
\def\ss{supersingular }
\def\Eisen{Eisenstein }
\def\pont{Pontryagin } % Pontryagin dual
\def\padic{\text{$p$-adic }}
\def\auto{\text{automorphic }}
\def\BS{Bruhat-Schwartz }
\def\GinKarp{\text{Gindikin-Karpelevi\v{c} }}
\def\Versch{\emph{Verschiebung }}
\def\Shord{\text{Schr\"{o}dinger }}
\def\Schordinger{\text{Schr\"{o}dinger }}
\def\SerreH{\text{Serre-Hochschild }}
\def\Teich{Teichm\"{u}ller }
\def\Neron{N\'{e}ron }
\def\Frob{\mathrm{Frob}}
% moduli notation
\def\mg{{\mathcal M}_g}
\def\agd{{\mathcal A}_{g,d}}
\def\Ag{\mathcal A}

% \cal, \frak, \mathbf.. check Math Sci.
% \mathcal, \mathfrak, \EuScript (euscript), \mathbb

% better notation
\newcommand{\per}{\bot}
\newcommand{\<}{\langle}   %\< is not defined yet.
\renewcommand{\>}{\rangle} %\> is already defined.
\def\then{\Rightarrow}
\def\oneone{\mbox{$\longleftrightarrow$}}  %\11 can't be used
\def\isoto{\stackrel{\sim}{\to}}
\def\isotoL{\stackrel{\sim}{\leftarrow}}
\def\surjto{\twoheadrightarrow}
\def\imply{\Rightarrow}
\def\ot{\otimes}
\def\boxt{\boxtimes}
\def\hookto{\hookrightarrow}
\def\longto{\longrightarrow}
\def\ol{\overline}  \nc{\opp}{\mathrm{opp}} \nc{\ul}{\underline}
\newcommand\bra[1]{[{#1}]}
%\nc{\embed}{\hookrightarrow}

%useful operators
\newcommand{\pair}[2]{\< #1, #2\>}
\newcommand{\bbpair}[2]{\<\!\<#1,#2\>\!\>}
\newcommand{\altpair}[2]{(#1,#2)}
\newcommand{\rpair}[2]{(#1,#2)}
\newcommand{\brpair}[2]{[ #1, #2]}
\newcommand{\pairing}{\pair{\,}{\,}}
\def\bbpairing{\bbpair{\,}{\,}}
\def\altpairing{\altpair{\,}{\,}}
\def\rpairing{\altpair{\,}{\,}}
\def\brpairing{\brpair{\,}{\,}}
\newcommand{\defil}[2]{{#1}_1\supset {#1}_2\supset\dots\supset {#1}_{#2}}
\newcommand{\defilo}[2]{{#1}_0\supset {#1}_1\supset\dots\supset {#1}_{#2}}
\newcommand{\infil}[2]{{#1}_1\subset {#1}_2\subset\dots\subset {#1}_{#2}}
\newcommand{\infilo}[2]{{#1}_1\subset {#1}_1\subset\dots\subset
  {#1}_{#2}}
% never number appeared in the newcommand name!

\newcommand{\stackunder}[2]{\raisebox{-1ex}{$\stackrel{\textstyle
#1}{\scriptstyle #2}$}}


%XY matrix notation
\def\XYmatrix{\xymatrix@M=8pt} % make \xymatrix not too cluttered
\def\ncmd{\newcommand}
\ncmd{\xysubset}[1][r]{\ar@<-2.5pt>@{^(-}[#1]\ar@<2.5pt>@{_(-}[#1]}
\ncmd{\XYmatrixc}[1]{\vcenter{\XYmatrix{#1}}}
\ncmd{\xyto}[1][r]{\ar@{->}[#1]}
\ncmd{\xyinj}[1][r]{\ar@{^(->}[#1]}
\ncmd{\xysurj}[1][r]{\ar@{->>}[#1]}
\ncmd{\xyline}[1][r]{\ar@{-}[#1]}
\ncmd{\xydotsto}[1][r]{\ar@{.>}[#1]}
\ncmd{\xydots}[1][r]{\ar@{.}[#1]}
\ncmd{\xyleadsto}[1][r]{\ar@{~>}[#1]}
\ncmd{\xyeq}[1][r]{\ar@{=}[#1]} \ncmd{\xyequal}[1][r]{\ar@{=}[#1]}
\ncmd{\xyequals}[1][r]{\ar@{=}[#1]}
\ncmd{\xymapsto}[1][r]{l\ar@{|->}[#1]}\ncmd{\xyimplies}[1][r]{\ar@{=>}[#1]}
\ncmd{\xyiso}{\ar[r]_-{\sim}}
\def\injxy{\ar@{^(->}}

%*************************Matrices
\newcommand{\Cln}[3]{\bbmx #1\\#2\\#3 \ebmx}

\newcommand{\mx}[4]{\begin{array}{cc}{#1}&
 {#2}\\{#3}&{#4}\end{array}}
\newcommand{\MX}[4]{\begin{bmatrix}
{#1}& {#2}\\
{#3}&{#4}\end{bmatrix} }

\newcommand{\pMX}[4]{\begin{pmatrix}
{#1}& {#2}\\
{#3}&{#4}\end{pmatrix} }

\newcommand{\bMX}[4]{\left[\begin{matrix}
{#1}&{#2}\\
{#3}&{#4}\end{matrix}\right]}

 \newcommand{\DII}[2]{\begin{bmatrix}{#1}&0
 \\0&{#2}\end{bmatrix}}
 \newcommand{\pDII}[2]{\begin{pmatrix}{#1}&0
 \\0&{#2}\end{pmatrix}}

\newcommand{\DIII}[3]{\begin{bmatrix}{#1}&&\\
&{#2}&\\
&&{#3}\end{bmatrix}}

\newcommand{\UPIII}[3]{\begin{bmatrix}1&{#1}&{#2}\\
&1&{#3}\\
&&1\end{bmatrix}}

\newcommand{\cln}[2]{\left[\begin{matrix}
  {#1} \\
  {#2}\\
\end{matrix}\right]
}
\newcommand{\xcln}[2]{\begin{matrix}
  {#1} \\
  {#2}\\
\end{matrix}
}
\newcommand{\xrow}[2]{\begin{matrix}
  {#1} &{#2}
\end{matrix}
}
\newcommand{\ADIII}[3]{\begin{bmatrix}
   &  &{#1}  \\
   &{#2} & \\
   {#3}&  &  \\
\end{bmatrix}}

\newcommand{\DIV}[4]{\begin{bmatrix}
{#1}&&&\\
&{#2}&&\\
&&{#3}&\\
&&&{#4}
\end{bmatrix}}



%Metaplectic group
\newcommand\Meta[2]{\left({#1},{#2}\right)}
\def\tj{\tilde{j}}
\def\wtSL{\widetilde{\SL}}
\newcommand{\seesaw}[4]{{#1}\ar@{-}[rd]\ar@{-}[d]&{#2}\ar@{-}[d]\\
{#3}\ar@{-}[ru]&{#4}}

%Duals
\newcommand\dual[1]{{#1}^{\!\vee}} %Dual
\newcommand\Pdual[1]{{#1}^*} %Pontragin dual
\newcommand\Cdual[2]{{#1}^D} %Cartier dual


% *** ENGLISH ABBREVIATIONS ****************************************

% Some words
\def\by{\text{ by }}
\def\where{\text{ where }}
\def\ie{i.e. }
\def\eg{\mbox{{\it e.g.} }}
\def\etc{\mbox{{\it et cetera} }}
\def\cf{\mbox{{\it cf.} }}
\def\loccit{\mbox{{\it loc.cit.} }}
\def\opcit{\mbox{{\it op.cit.} }}
\def\can{{can}}
\def\etal{\mbox{{ et al.}}}
\def\resp{resp.$\,$}


%\renewcommand{\O}{\cO}
\def\wht#1{\widehat{#1}}
\def\Cyc{{\langle\varepsilon\rangle}}%universal deformation of cyclotomoic character
%\newcommand{\deform}[1]{\tilde{{#1}}}

%Category
\def\ENS{\mathfrak E\mathfrak n\mathfrak s}
\def\SCH{\mathfrak S\mathfrak c\mathfrak h}

% for extending arrows
\def\ext{\rule[.5ex]{5mm}{.1mm}}
\def\EXt{\rule[.5ex]{10mm}{.1mm}}
\def\back{\!\!\!}
\def\Back{\back\back}
% right surjective maps
\def\onsuffix{\longrightarrow\back\back\!\rightarrow}

\def\maponR{\smash{\mathop{\onsuffix}}}
\def\maponRR{\smash{\mathop{\ext\back\onsuffix}}}
\def\maponRRR{\smash{\mathop{\EXt\back\onsuffix}}}

\def\MaponR#1#2{\smash{\mathop{\onsuffix}\limits^{#1}_{#2}}}
\def\MaponRR#1#2{\smash{\mathop{\ext\back\onsuffix}\limits^{#1}_{#2}}}
\def\MaponRRR#1#2{\smash{\mathop{\EXt\back\onsuffix}\limits^{#1}_{#2}}}

% right maps
\def\mapR{\smash{\mathop{\longrightarrow}}}
\def\mapRR{\smash{\mathop{\ext\back\longrightarrow}}}
\def\mapRRR{\smash{\mathop{\Ext\back\longrightarrow}}}

\def\MapR#1#2{\smash{\mathop{\longrightarrow}\limits^{#1}_{#2}}}
\def\MapRR#1#2{\smash{\mathop{\ext\back\longrightarrow}\limits^{#1}_{#2}}}
\def\MapRRR#1#2{\smash{\mathop{\Ext\back\longrightarrow}\limits^{#1}_{#2}}}

% right injective maps
\def\inprefix{\mbox{\raisebox{1mm}{\tiny $\subset$}}\!\!}

\def\mapinR{\smash{\mathop{\inprefix\!\!\longrightarrow}}}
\def\mapinRR{\smash{\mathop{\inprefix\ext\back\longrightarrow}}}
\def\mapinRRR{\smash{\mathop{\inprefix\Ext\back\longrightarrow}}}

\def\MapinR#1#2{\smash{\mathop{\inprefix\!\!\longrightarrow}\limits^{#1}_{#2}}}
\def\MapinRR#1#2{\smash{\mathop{\inprefix\ext\back\longrightarrow}\limits^{#1}_{#2}}}
\def\MapinRRR#1#2{\smash{\mathop{\inprefix\Ext\back\longrightarrow}\limits^{#1}_{#2}}}

% exact sequence
\newcommand{\exact}[3]{
0\mapR{#1}\mapR{#2}\mapR{#3}\mapR 0 }
\newcommand{\Exact}[5]{
0\mapR{#1}\MapR{#2}{} {#3}\MapR{#4}{} {#5}\mapR 0 }

\newcommand{\edit}[1]{\footnote{#1}\marginpar{\hfill {\sf\thefootnote}}}
\newcommand{\todo}[1]{\noindent$\bullet$ {\small \textsf{#1}} $\bullet$\\}
\newcommand{\done}[1]{\noindent {\small \textsf{Done: #1}}\\}
\newcommand{\danger}[1]{\marginpar{\small \textsl{#1}}}

% characteristic function of a set
\def\Ch{\mathrm{char}}
%\newcommand{\ch}{characteristic }
\def\ch{{\mathbb I}}

\def\hb#1{\hbox{ #1}}

%Local fields
\def\uf{\varpi} %uniformizer
\def\Abs{{|\!\cdot\!|}} %adelic absolute value
%\providecommand\abs[1]{\lvert{#1}\rvert}

% Control symbols
\newcommand{\npr}{\noindent }
\newcommand{\pr}{\indent }


% abbreviation
\def\Sg{{\varSigma}}  %%CM type
\def\Sgbar{\Sg^c}
\def\ndivides{\nmid}
\def\ndivide{\nmid}
\def\x{{\times}}
\def\xx{\,\times\,}
\def\tame{\mathrm{tame}}
\def\onehalf{{\frac{1}{2}}}
\def\e{\varepsilon} % episilon factor
\def\al{\alpha}
\def\Beta{\boldsymbol \beta}
\def\Lam{\Lambda}
\def\kap{\kappa}
\def\om{\omega}
\def\dirlim{\varinjlim}
\def\prolim{\varprojlim}
\def\iso{\simeq}
\def\con{\equiv}
\def\bksl{\backslash}
\newcommand\stt[1]{\left\{#1\right\}}
\def\ep{\epsilon}
\def\varep{\varepsilon}
\def\l{{\ell}}
\def\pd{\partial}
\def\lam{\lambda}
\def\AI{\textrm{AI}} % automotphic induction
\def\pii{\pi i}
\def\hot{\widehat{\ot}}
\def\half{\frac{1}{2}}
\def\Ups{\Upsilon}
\def\cpd{2\pi i}
\def\vep{\varepsilon}
\def\ka{\kappa}
\def\sg{\sigma}
\def\vp{\varphi}
\def\disjoint{\sqcup}
\def\bigot{\bigotimes}
\def\Pol{\mathrm{Pol}}
\def\smid{\,|}

%Symbol for measures
\def\dx{{\rm d}^\x}
\def\dxx{{\rm d}^\x x}
\def\dxv{dx_v}
\def\dxp{dx_p}
\def\dd{{\rm d}}

% ideles and adeles
\def\Adele#1{#1(\Q)\bksl #1(\A)}
\def\idele{\A^\times}
\def\AFf{\A_{\cF,f}}
\def\AKf{\A_{\cK,f}}
\def\AF{\A_\cF}
\def\AK{\A_\cK}
\def\setp{{(p)}}
\def\setinfp{{(\infty,p)}}
\def\setinf{{(\infty)}}
\def\bbox{{(\Box)}}

\newcommand{\powerseries}[1]{\llbracket{#1}\rrbracket}
\newcommand{\formal}[1]{\widehat{#1}}
\renewcommand\pmod[1]{\,(\mbox{mod }{#1})}
\renewcommand\mod[1]{\,\mbox{mod }{#1}}
\newcommand\PD[1]{\frac{\partial}{\partial{#1}}}
%\newcommand\DD[2]{\frac{\partial{#1}}{\partial{#2}}}
\renewcommand\Re{\text{Re}\,}
\newcommand\Dmd[1]{\left<{#1}\right>} %Diamond operator
\def\vphi{\varphi}
\def\Her{\EucH} %Hermitian matrix
\def\Cp{\C_p}
\def\inert{{\mathrm{inert}}}
\def\ram{{\mathrm{ram}}}
\def\split{{\mathrm{split}}}
\def\alg{\mathrm{alg}} 
\def\Qq{\Q_q} 
\def\pmq{q}
\def\cond{{\rm cond}}


